Fast and Robust Distributed Learning in High Dimension

Could a gradient aggregation rule (GAR) for distributed machine learning be both robust and fast? This paper answers by the affirmative through multi-Bulyan. Given $n$ workers, $f$ of which are arbitrary malicious (Byzantine) and $m=n-f$ are not, we prove that multi-Bulyan can ensure a strong form of Byzantine resilience, as well as an ${\frac{m}{n}}$ slowdown, compared to averaging, the fastest (but non Byzantine resilient) rule for distributed machine learning. When $m \approx n$ (almost all workers are correct), multi-Bulyan reaches the speed of averaging. We also prove that multi-Bulyan's cost in local computation is $O(d)$ (like averaging), an important feature for ML where $d$ commonly reaches $10^9$, while robust alternatives have at least quadratic cost in $d$. Our theoretical findings are complemented with an experimental evaluation which, in addition to supporting the linear $O(d)$ complexity argument, conveys the fact that multi-Bulyan's parallelisability further adds to its efficiency.

==> cost.tex <==
\paragraph{Cost analysis.}
Our empirical results are consistent with the complexity of the algorithmic components of \system.

The model update time complexity\footnote{If not stated otherwise, we refer to the worst-case time complexity.} of both \systemA and \systemB is $\bigO(n^2d)$.
This is essentially the same as a baseline $GAR$-based SGD algorithm, i.e., averaging\footnote{Averaging is not Byzantine-resilient.} when $d >> n$ (valid assumption for modern ML).
\systemB induces an additional overhead of $\bigO(nd)$ (coordinate-wise median) on top of $n-2f$ executions of \systemA, leading to a total model update complexity of $\bigO(nd + f\cdot nd) = \bigO(n^2d)$.
We conjecture that $\Omega(n^2d)$ is a lower bound for every weakly Byzantine-resilient SGD algorithms.
\system is strongly Byzantine-resilient with the same complexity.

Baseline averaging SGD requires $\bigO(\frac{1}{\sqrt{nb}})$ steps to converge.
In other words SGD goes as fast as permitted by the square root of the total number of samples used per step.
The more samples, the lower the variance and the better the gradient estimation (the closer are the black arrows to the blue arrow in Figure~\ref{fig:byzbehavior}).

Everything else being equal (mini-batch sizes, smoothness of the cost function etc), and in the absence of Byzantine workers, the number of steps required for \system to converge is $\bigO(\frac{1}{\sqrt{m}})$.
The higher the value of $m$ the fewer steps required for convergence.
The temptation is then to increase $m$ to the highest value possible, so that there are fewer steps required to converge.
We derive the maximum possible value for $m$ that ensures weak Byzantine resilience, $\tilde m=n-2f-2$\footnote{A higher value of $n-f-2$ for $m$ can be selected if only weak Byzantine resilience is required and only \systemA is used.}~\cite{proofs}.
We also prove that this will induce a slowdown of $\Omega(\sqrt{\frac{\tilde m}{n}})$ (always computed as the ratio between \system and averaging), in the absence of Byzantine workers.
In other words, $\tilde m$ enables the fastest convergence while still ensuring the safety requirement of Byzantine resilience.

